Dense X Retrieval: What Retrieval Granularity Should We Use?

Dense retrieval has become a prominent method to obtain relevant context or world knowledge in open-domain NLP tasks. When we use a learned dense retriever on a retrieval corpus at inference time, an often-overlooked design choice is the retrieval unit in which the corpus is indexed, e.g. document, passage, or sentence. We discover that the retrieval unit choice significantly impacts the performance of both retrieval and downstream tasks. Distinct from the typical approach of using passages or sentences, we introduce a novel retrieval unit, proposition, for dense retrieval. Propositions are defined as atomic expressions within text, each encapsulating a distinct factoid and presented in a concise, self-contained natural language format. We conduct an empirical comparison of different retrieval granularity. Our experiments reveal that indexing a corpus by fine-grained units such as propositions significantly outperforms passage-level units in retrieval tasks. Moreover, constructing prompts with fine-grained retrieved units for retrieval-augmented language models improves the performance of downstream QA tasks given a specific computation budget.

==> sections/analysis.tex <==


\section{Analysis and Discussion}

In this section, we discuss where and why retrieval by prop has advantage over sentence and passage.
We find retrieval by proposition has a better generalization under query shift (\cref{sec:generalization}), and has a higher attention to long-tail entity (\cref{sec:longtail}). We also find the retrieved propositions as a higher question-related information density compared to sentences and passages (\cref{sec:density}).


% \subsection{Choosing decomposition method}
% - 1\% dataset (400k paragraph)

% 1. only proposition segments 
% 2. only decontextulization

% sentence-level rule-based decomposition
% sentence-level decomposition
% sentence decontextulization (without decomposition)
% ours

% We hypothesize decontextulization contribute necessary context to match the user's query. Without necessary context, the performance of both in-domain and out-of-domain queries will decrease. Decomposition make the document semantically similar to the user's query. Without decomposition, the performance of out-of-domain decrease.  

% \subsection{Distillation}

% [mt0, t5-base, t5-large, t5-3b]
% [gpt-3.5, gpt-4] x 100k

% We hypothesize that more training data and larger model can fit the training data better.

% [t5-large] x [gpt-3.5, gpt-4] x [6 dataset] x 6 models

% We hypothesize that the decomposition model distilled from 1-shot GPT-4 is better than 1-shot GPT-3.5.

% \subsection{Case study of the decomposition qulities}


